A Disparity Refinement Framework for Learning-based Stereo Matching Methods in Cross-domain Setting for Laparoscopic Images

Purpose: Stereo matching methods that enable depth estimation are crucial for visualization enhancement applications in computer-assisted surgery (CAS). Learning-based stereo matching methods are promising to predict accurate results on laparoscopic images. However, they require a large amount of training data, and their performance may be degraded due to domain shifts. Methods: Maintaining robustness and improving the accuracy of learning-based methods are still open problems. To overcome the limitations of learning-based methods, we propose a disparity refinement framework consisting of a local disparity refinement method and a global disparity refinement method to improve the results of learning-based stereo matching methods in a cross-domain setting. Those learning-based stereo matching methods are pre-trained on a large public dataset of natural images and are tested on two datasets of laparoscopic images. Results: Qualitative and quantitative results suggest that our proposed disparity framework can effectively refine disparity maps when they are noise-corrupted on an unseen dataset, without compromising prediction accuracy when the network can generalize well on an unseen dataset. Conclusion: Our proposed disparity refinement framework could work with learning-based methods to achieve robust and accurate disparity prediction. Yet, as a large laparoscopic dataset for training learning-based methods does not exist and the generalization ability of networks remains to be improved, the incorporation of the proposed disparity refinement framework into existing networks will contribute to improving their overall accuracy and robustness associated with depth estimation.

==> draft.tex <==
\begin{document}

% hence it supports further applications such as scene understanding, object detection, odometry, and SLAM

% Pixel to pixel correspondences can be found from a stereo image pair via stereo matching techniques. matched pixels can be triangulated

% The recovery of 3D information from stereo images is one of the classic problems in
% computer vision



% The current state of stereo matching

% Very limited.

% Current state of stereo matching, dataset. 

% In this section, we briefly survey relevant stereo-matching
% methods. For a comprehensive review for stereo-matching,
% please see the references therein.

% This section mainly focuses 

% The dissimilarity measure used
% during propagation is the zero mean normalized cross correlation (ZNCC), which is
% less prone to illumination bias in homogeneous regions while it is also more indicative in regions with discriminative texture.

% Stereo
% matching is an important and active topic in the computer
% vision field and a large number of effective methods exist,
% and reader may refer to the Middlebury website [12] for the
% list of stereo matching methods. 



% 1. \cite{stoyanov2010real} we present a novel stereo reconstruction algorithm that propagates disparity information around a set of candidate feature matches.  semi-dense.  Feature Matching.
% Stoyanov et al. [22] and Chang [23] matched a sparse set
% of salient regions using stereo Lucas-Kanade and propagated
% the disparity around each matched region.

% This has the advantage of
% avoiding problems with specular highlights, occlusions from instruments and
% view dependent illumination bias.

% ELAS uses Sobel masks to conduct sparse corners matching as the supporting points set. Then, the
% aligned sparse supporting points are triangulated to generate
% prior pixel-wise disparity. Finally, the maximum a-posteriori
% (MAP) algorithm is adopted to estimate the optimal dense
% disparity. T

% 2. LEAS \cite{geiger2010efficient} is also popular. is still one of the most widely
% used stereo matching algorithms due to its robustness and
% accuracy


% To provide an acceptable initialization, Revaud et al. [36]
% proposed the use of a structure edge detection approach [37]
% for feature point detection and DeepMatching [38] for feature
% matching, to create an initialization to compute the optical
% flow. Bao et al. [39] proposed an improved non-local patch
% matching technique with a bilateral weighted matching cost
% for large displacement optical flow

% variational optimization methods

% they are limited
% by image characteristics including illumination differences,
% weak texture content, specular highlights, and occlusions.
% To overcome these limitations, 

% An initial disparity map is first estimated by linearly
% interpolating these disparity values of matched feature points
% across the scan-line. Then the initial disparity map Dˆ can be
% further smoothed by using the weighted median filter with
% bilateral weights [44].

% method for laparoscopic images, comprising an efficient sparse-dense feature matching step, left and right image illumination equalization, and
% refined disparity optimization. 

% We propose a solution with very low time complexity and competitive accuracy for the computation of dense optical
% flow. It consists of three parts: (1) inverse search for patch correspondences; (2) dense displacement field creation through patch aggregation
% along multiple scales; (3) variational refinement. At the core of our Dense
% Inverse Search-based method (DIS) is the efficient search of correspondences inspired by the inverse compositional image alignment proposed by
% Baker and Matthews (2001, 2004). 

% 4. \cite{kroeger2016fast},\cite{song2021bayesian}. Inverse Search-based method (DIS) 
%  (1) inverse search for patch correspondences; (2) dense displacement field creation through patch aggregation along multiple scales; (3) variational refinement.
 
 
% SGM and LEAS are two major methods used SLAM
% Local:  SGM \cite{hirschmuller2005accurate},\cite{zhang2020template}, , 
 
% The overlapping
% image patches (arbitrary squared image segment) from the
% images at different scales are aligned based on the photometric
% consistency presumption. We propose a Bayesian framework
% to evaluate the probability of the optimized patch disparity
% at different scales. 

% , they require both
% good disparity initialization, as well as input images that have
% been equalized with respect to illumination for the linearization to be effective, especially for scenes with large disparities.
% To provide an acceptable initialization,
% \textbf{}


% The recovery of 3D information from stereo images is one of the classic problems in
% computer vision. Recent review articles provide a good summary of progress in the field [3, 4] and establish a benchmarking framework with ground truth data [3]. Stereo
% matching is an important and active topic in the computer
% vision field and a large number of effective methods exist,
% and reader may refer to the Middlebury website [12] for the
% list of stereo matching methods.

% A large volume of studies on stereo matching have been published; we review the closely related literature.



% In this work, we relied on reasonable assumptions

% \cite{yan2019segment}: one is the MRF inference which is able to estimate mean disparities
% of superpixels as well as the mean disparities of occluded
% regions, and the other is the Bayesian inference based disparity
% plane refinement which generates a smooth disparity map.
% Experiments demonstrate the good performance in occlusion
% handling with low computational cost.

% 1. not in cross domain setting. 2. only one network. 3. smooth and not deal large area of pitfalls can not be directly refined. 4. prior knowledge/assumption have not been exploited.

% Considering 1.ground truth

% It is shown [16] that multi-step and
% iterative refinement strategies can result in competitive results.
% However, in large occluded regions, inner occlusions cannot
% be directly refined by these strategies and cumulative error
% may be introduced. However, in terms of endoscopic images, prior assumption should be exploited. They are not designed for endoscopic images.

% Thus, we propose
% a multistep refinement to identify and correct the outliers.
% Different from the above-mentioned methods, we classify the
% outliers into leftmost and inner kinds, and different approaches
% are taken to recover the outliers according to their kinds.
% Moreover, the image-guided exponential step filter further
% optimizes the disparity map.

% To detect outliers, confidence measures \cite{poggi2021confidence} are conducted on the disparity map.


%Huang and Zhang [14] proposed a fast refinement including belief aggregation for outlier %detection and belief propagation for filling.

% minimum spanning tree

% Most refinement methods follow the detection
% and filling scheme, followed by a filtering step. Left-right
% consistency check (LRC) [11] is commonly used to detect
% outliers.

% To achieve higher accuracy, refinement is undertaken to identify and correct the outliers in the
% raw disparity map. Left–right consistency (LRC) checking [1]
% is the widely used method to detect the outliers. The detection
% method in [11] provided a way to distinguish the occluded outliers and the mismatched outliers. Several approaches, including region voting [19], vertical voting [20], cost spectrum peak
% analysis and removal [30], subpixel enhancement [19], [31],
% as well as filtering methods (e.g., using median filtering and
% weighted median filter [6], [7]), aimed at correcting the outliers
% in the raw disparity map. All the methods have flaws, and
% no single one method can remove all the outliers. Therefore,
% multistep refinement is adopted in [17], [19], and [31] to
% systematically remove outliers. This strategy achieved competitive results according to the literature. Thus, we propose
% a multistep refinement to identify and correct the outliers.
% Different from the above-mentioned methods, we classify the
% outliers into leftmost and inner kinds, and different approaches
% are taken to recover the outliers according to their kinds.
% Moreover, the image-guided exponential step filter further
% optimizes the disparity map.

% Occlusion

% Usually follow outlier detection and refinement, including.....

% However deep learning end to end fashion, evaluated on the same domain and achieve very good results.

% Disparity refinement is designed to further improve the
% results in hard regions, such as occluded regions and low
% texture regions. 

% real-time processing on CPU.

% Refinement detection and refinement. 

% These errors are usually concentrated in uniform texture-less areas, half-occlusions and regions near depth discontinuities. One way of dealing with stereo-matching errors is to use various techniques of detecting potentially inaccurate disparity values and invalidate them, therefore making the disparity map semi-sparse. Several such techniques are already implemented in the StereoBM and StereoSGBM algorithms. Another way would be to use some kind of filtering procedure to align the disparity map edges with those of the source image and to propagate the disparity values from high- to low-confidence regions like half-occlusions. Recent advances in edge-aware filtering have enabled performing such post-filtering under the constraints of





%Above mentioned
%Domain adaptation. GAN \cite{mahmood2018unsupervised}, module.



% For all methods mentioned above, the computed disparity
% maps often have streak-like artifact and are not smooth in
% general. Thus, post-processing steps including left-right consistency check [40], [41], super-pixel interpolation [24], [42],
% and weighted median filtering [19], [43], [44] are often applied
% to the computed disparity map in order to remove these streaklike artifacts and to promote the computation of a smooth
% disparity map.

% Artifacts will violate some assumptions

% We also included PSMNET despite its slower performance
% since this was the winning technique of a grand challenge
% in endoscopic video.
%  correlation-based AANet [39],
% 3D convolution-based PSMNet [5] 

% Concurrently, networks such as [20, 5] build a 4D feature volume by concatenating features at different disparities and learn to compute/aggregate the matching cost by
% 3D convolutions.

%was the winning technique of a grand challenge
% in endoscopic video.

% popular and winner.  3D convolutions for cost aggregation and accordingly obtains better accuracy

% The stacked hourglass 3D CNN
% repeatedly processes the cost volume in a top-down/bottomup manner to further improve the utilization of global context information.

% To this end, a motivating question arises: How to achieve
% state-of-the-art results without any 3D convolutions while
% being significantly faster? Answering this question is especially challenging due to the strong regularization provided
% by 3D convolutions. In this paper, we show that by designing two effective and efficient modules for cost aggregation, competitive performance can be obtained on both
% Scene Flow and KITTI datasets even with simple feature
% correlation [20] instead of concatenation

% In this paper, we aim at completely replacing the commonly used 3D
% convolutions to achieve fast inference speed while maintaining comparable accuracy. To this end, we first propose a sparse points based intra-scale cost aggregation
% method to alleviate the well-known edge-fattening issue at
% disparity discontinuities. Further, we approximate traditional cross-scale cost aggregation algorithm with neural
% network layers to handle large textureless regions. Both
% modules are simple, lightweight, and complementary, leading to an effective and efficient architecture for cost aggregation.

% a new end-to-end-trained stereo depth estimation network based on the current Transformer architecture [36] presented for language processing and recent breakthroughs in feature matching [31]. (STTR).

% We report promising results on both synthetic and real-world datasets and
% demonstrate that STTR generalizes across different domains, even without fine-tuning.

% We take advantage of the recent Transformer architecture [36] proposed for language processing
% and recent advances in feature matching [31], and present
% a new end-to-end-trained stereo depth estimation network
% named STereo TRansformer (STTR). Synthetic and real-world datasets and
% demonstrate that STTR generalizes across different domains, even without fine-tuning.

%  deep stereo matching networks

% we propose the first end-to-end hierarchical NAS framework for deep
% % stereo matching 

% Neural Architecture Search

% LEAStereo [7] is further optimized within this
% structure using neural architecture search, top performance.

% Extensive experiments show that our searched network outperforms all state-of-the art deep stereo matching architectures and is ranked at the top 1 accuracy on KITTI
% stereo 2012, 2015 and Middlebury benchmarks, as well as the top 1 on SceneFlow
% dataset with a substantial improvement on the size of the network and the speed of
% inference. 

% To reduce the human efforts in neural network design, Neural Architecture Search
% (NAS) has been applied with remarkable success to various high-level vision tasks
% such as classification and semantic segmentation. The underlying idea for the
% NAS algorithm is straightforward, namely, to enable the network the ability to
% choose among a set of operations (e.g.,convolution with different filter sizes), one
% is able to find an optimal architecture that is better adapted to the problem at hand.
% However, so far the success of NAS has not been enjoyed by low-level geometric
% vision tasks such as stereo matching. This is partly due to the fact that state-ofthe-art deep stereo matching networks, designed by humans, are already sheer in
% size. Directly applying the NAS to such massive structures is computationally
% prohibitive based on the currently available mainstream computing resources. In
% this paper, we propose the first end-to-end hierarchical NAS framework for deep
% stereo matching by incorporating task-specific human knowledge into the neural
% architecture search framework. 


% Fig.1. Illustration of pitfalls. textureless regions, occlusion, specular highlights, and domain shift.

% The pipeline is depicted in Fig.2. 

% matching errors.

% Deep learning methods [5, 17, 21, 45, 48] work extremely well on disparity estimation when sufficient data with ground truth are available. However, they have been
% proven vulnerable to out-of-distribution data. When dealing
% with unseen environments quite different from those employed to train the network, the accuracy may rapidly decrease.

% Motivating Example.
% Here it is evident that fine tuning on real images is not sufficient to obtain reliable performance across all environments as evidenced by the major mistakes in (c) marked in white.
% As can be seen, (c) behaves worse than the network trained only on synthetic data and adapted online to the target domain in an unsupervised manner by our formulation (d).


% Stereo matching algorithms, especially highly-optimized ones that are intended for real-time processing on CPU, tend to make quite a few errors on challenging sequences. These errors are usually concentrated in uniform texture-less areas, half-occlusions and regions near depth discontinuities. One way of dealing with stereo-matching errors is to use various techniques of detecting potentially inaccurate disparity values and invalidate them, therefore making the disparity map semi-sparse. Several such techniques are already implemented in the StereoBM and StereoSGBM algorithms. Another way would be to use some kind of filtering procedure to align the disparity map edges with those of the source image and to propagate the disparity values from high- to low-confidence regions like half-occlusions. Recent advances in edge-aware filtering have enabled performing such post-filtering under the constraints of real-time processing on CPU.


% Interpolation is performed by
% propagating valid disparities through neighboring invalid
% disparity areas. 

% This is done similarly to SGM along paths
% from eight directions. For each invalid pixel, all eight
% values v pi are stored. The final disparity image D 0 is created by:


% For each invalid pixel, all eight values v pi are stored.
% eight directions.

% Interpolation is performed by
% propagating valid disparities through neighboring invalid
% disparity areas.

% Outliers are selected 


% from $C_f(\mathbf{x})$


% We binarize the $C_f(\mathbf{x})$ with the threshold $th_f$


% \subsubsection{Interpolation from Neighboring Disparities}



% ded for real-time processing on CPU, tend to make quite a few errors on challenging sequences. These errors are usually concentrated in uniform texture-less areas, half-occlusions and regions near depth discontinuities. One way of dealing with stereo-matching errors is to use various techniques of detecting potentially inaccurate disparity values and invalidate them, therefore making the disparity map semi-sparse.

%assess
%analysis
% we further demonstrate
% depict organ/specular highlight/uneven illumination/spikes/holes/
%produce, despite
%estimate
%generate
%defects
% yield degraded
% spikes holes
% robust
% summarize the results of the quantitative assessment 
% Numerical results are summarised

% We conduct ablation studies using the Scene Flow synthetic dataset, and provide quantitative results for the effects
% of the attention mask, optimal transport layer, context adjustment layer and positional encoding summarized in Table 1. Following prior work, we validate on the test split
% directly since Scene Flow is only used for pre-training.

% We conduct an ablation study to analyze the performance of each pipeline component to determine the contribution brought forth by each of the separate components integrated into our proposed pipeline. 
% To determine the value added by each of the different components that make up our proposed pipeline,
% We conduct three comparative experiments to understand the benefits.

% a robust depth prior and
% gives reasonable depth prediction to assist a SLAM system.
% 2

% This makes the bootstrapping stage much faster and more stable.
% In fact, many SLAM systems cannot even bootstrap for challenging
% tasks such as colonoscopy

% 1. Require more level,time running.
% GDR robust to those problems.
% 2. make LR good.
% GL require good initialization.
% Saves time.
% Boost stripping effect achieved.
% SDR 1.17944 second.




% \subsection{Test}


% ded for real-time processing on CPU, tend to make quite a few errors on challenging sequences. These errors are usually concentrated in uniform texture-less areas, half-occlusions and regions near depth discontinuities. One way of dealing with stereo-matching errors is to use various techniques of detecting potentially inaccurate disparity values and invalidate them, therefore making the disparity map semi-sparse.

%assess
%analysis
% we further demonstrate
% depict organ/specular highlight/uneven illumination/spikes/holes/
%produce, despite
%estimate
%generate
%defects
% yield degraded
% spikes holes
% robust
% summarize the results of the quantitative assessment 
% Numerical results are summarised


% Two figures.
% 3D point cloud.


% percentage of
% pixels with disparity error larger than 3 (bad3) as suggested
% in [3], [4]. 

% \subsection{Comparison with other Descriptors}
% Illumination invariant.


% \begin{table*}[htpb]
%     \centering
%     \caption{Result.}
%     \resizebox{0.99\linewidth}{!}{%
%     \begin{tabular}{||c||c|c||c|c||c|c||}
%     \hline
%      & \multicolumn{2}{c||}{Occlusions included} % ($1024\times1280$)
%      & \multicolumn{2}{c||}{Occlusions not included}  %($512\times512$)
%      %& \multicolumn{3}{c||}{SCARED} %($576\times720$) \\%
%     \\% \cline{2-10}
%     %\hline
%       & RMSE Disparity (pixel)  & RMSE Depth (mm) 
%      & RMSE Disparity (pixel)  & RMSE Depth (mm)   \\ \hline 
%   D1  
%     % & 16.14 $\pm$ 3.45 & 16.08 $\pm$ 3.16 & 12.72
%   & 8.3789 $\pm$ 7.07926 & 48.6295 $\pm$ 150.328 & 5.69599 $\pm$ 4.75148 & 6.91667 $\pm$ 5.07809 \\
%   Path-Intensity  
%     % & 16.14 $\pm$ 3.45 & 16.08 $\pm$ 3.16 & 12.72
%   & 47.2425 $\pm$ 9.51323 & 772.829 $\pm$ 261.629 & 38.8349 $\pm$ 9.13431 & 741.07 $\pm$ 226.874 \\
%   \hline
%     \end{tabular}
%     }%
%     \label{tab:generalization}
% \end{table*}

\end{document}
